Efficient Backpropagation with Variance-Controlled Adaptive Sampling

Sampling-based algorithms, which eliminate ''unimportant'' computations during forward and/or back propagation (BP), offer potential solutions to accelerate neural network training. However, since sampling introduces approximations to training, such algorithms may not consistently maintain accuracy across various tasks. In this work, we introduce a variance-controlled adaptive sampling (VCAS) method designed to accelerate BP. VCAS computes an unbiased stochastic gradient with fine-grained layerwise importance sampling in data dimension for activation gradient calculation and leverage score sampling in token dimension for weight gradient calculation. To preserve accuracy, we control the additional variance by learning the sample ratio jointly with model parameters during training. We assessed VCAS on multiple fine-tuning and pre-training tasks in both vision and natural language domains. On all the tasks, VCAS can preserve the original training loss trajectory and validation accuracy with an up to 73.87% FLOPs reduction of BP and 49.58% FLOPs reduction of the whole training process. The implementation is available at https://github.com/thu-ml/VCAS .

==> src/apppendix-notations.tex <==
\section{Notations}
In this section, we will explain the notations of this work in detail.
\begin{table}[!h]
    \centering
    \caption{Notations}
    \label{tab:notation}
    \begin{threeparttable}
    % \resizebox{\textwidth}{!}{
    \begin{tabular}{p{0.08\textwidth}c}
        \toprule
        Notation & Meanings \\
        \midrule
        \underline{a} \\
        \bottomrule
    \end{tabular}
    % }
    \end{threeparttable}
\end{table}

% \begin{table}[h]
% \caption{Notation des SCLSP-RM\textsuperscript{gen} Modells nach Sahling et all.(2016)}
% \begin{tabularx}{\textwidth}{p{0.08\textwidth}X}
% \toprule
  
%   \multicolumn{2}{l}{{\ul Indices:}}                                       \\
%   $K$ & number of products (k \in\{1,...,K\})  \\ 
%   $T$ & number of periods (t \in\{1,...,T\})\\
  
%   \multicolumn{2}{l}{{\ul Parameters:}}                                       \\  
%   \delta_k & target δ-service level for product k \\
%   \epsilon &  \\
%   c_t      & production capacity in period t \\
%   c^r_t    & Remanufacturing capacity in period t  \\
%   hc_k     & holding cost of product k per unit and period   \\
%   hc_k     & holding cost of product k per unit and period   \\
%   oc   & overtime costs per unit   \\
%   M_{kt}   & bignumber for product k in period t\\
%   pc_{k}   & production cost of product k per unit\\
%   pc^r_{k} & remanufacturing cost of product k per unit\\
%   sc_{k}   &  setup cost of product k\\
%   sc^r_{k} &  setup cost of returned product k\\
%   tp_{k}   &  production time for one unit of product k\\
%   tp^r_{k} & remanufacturing time for one unit of product k\\
%   ts_{k}   & setup time of product k\\
%   ts^r_{k} & setup time of returned product k\\
  
%   \multicolumn{2}{l}{{\ul Random variables:}}                                       \\ 
%   BL_{kt}  & backlog of product k at the end of period t\\
%   D_{kt}   & external demand of product k in period t  \\
%   I_{kt}   & net inventory of product k at the end of period t  \\
%   I^r_{kt} & net inventory of returns of product k at the end of period t  \\
%   IP_{kt}   & physical inventory of product k at the end of period t\\
%   IP^r_{kt}   & physical inventory of recoverables at the end of period t\\
%   R_{kt}   &  returns of product k in period t\\
%   SF^r_{kt}   &  Shortfall of recoverables of product k in period t\\
  
%   \multicolumn{2}{l}{{\ul Decision variables:}}                                       \\
%   q_{kt}   &  production quantity of product k in period t\\
%   q^r_{kt}   &  remanufacturing quantity of product k in period t  \\
%   o_{t}   &  amount of overtime for production in period t  \\
%   o^r_{t}   &  amount of overtime for remanufacturing in period t\\
%  % \gamma_{kt}   &   binary setup indicator for production of product k in period t\\
%  % \gamma^r_{kt}   &  binary setup variable for remanufactured product k in period t\\
%   \bottomrule
%  \end{tabularx}
% \end{table}
